The angular momentum of baryons and dark matter halos revisited

Recent theoretical studies have shown that galaxies at high redshift are fed by cold, dense gas filaments, suggesting angular momentum transport by gas differs from that by dark matter. Revisiting this issue using high-resolution cosmological hydrodynamics simulations with adaptive mesh refinement, we find that at the time of accretion, gas and dark matter do carry a similar amount of specific angular momentum, but that it is systematically higher than that of the dark matter halo as a whole. At high redshift, freshly accreted gas rapidly streams into the central region of the halo, directly depositing this large amount of angular momentum within a sphere of radius r=0.1rvir. In contrast, dark matter particles pass through the central region unscathed, and a fraction of them ends up populating the outer regions of the halo (r/rvir>0.1), redistributing angular momentum in the process. As a result, large-scale motions of the cosmic web have to be considered as the origin of gas angular momentum rather than its virialised dark matter halo host. This generic result holds for halos of all masses at all redshifts, as radiative cooling ensures that a significant fraction of baryons remain trapped at the centre of the halos. Despite this injection of angular momentum enriched gas, we predict an amount for stellar discs which is in fair agreement with observations at z=0. This arises because the total specific angular momentum of the baryons remains close to that of dark matter halos. We propose a new scenario where gas efficiently carries the angular momentum generated by large-scale structure motions deep inside dark matter halos, redistributing it only in the vicinity of the disc.

==> PaxHeader/ms.tex <==
17 gid=784332012
18 uid=1289638921
20 ctime=1307058156
20 atime=1307058167
24 SCHILY.dev=234881027
23 SCHILY.ino=13999395
18 SCHILY.nlink=1

